Focusing on the Big Picture: Insights into a Systems Approach to Deep Learning for Satellite Imagery

Deep learning tasks are often complicated and require a variety of components working together efficiently to perform well. Due to the often large scale of these tasks, there is a necessity to iterate quickly in order to attempt a variety of methods and to find and fix bugs. While participating in IARPA's Functional Map of the World challenge, we identified challenges along the entire deep learning pipeline and found various solutions to these challenges. In this paper, we present the performance, engineering, and deep learning considerations with processing and modeling data, as well as underlying infrastructure considerations that support large-scale deep learning tasks. We also discuss insights and observations with regard to satellite imagery and deep learning for image classification.

==> DeepLearningFrameworksSubsection.tex <==
\subsubsection{Deep learning}
Many popular deep learning frameworks now exist in the open-source community for research and production purposes. TensorFlow\footnote{https://www.tensorflow.org/}, Keras\footnote{https://keras.io/}, and PyTorch\footnote{http://pytorch.org/}, and many others are popular frameworks with large open-source and industrial backings.
%
%\begin{itemize}
%	\item Ease of creating custom architectures
%	\item Ability to write custom loss functions and optimization strategies
%	\item Simple GPU acceleration
%\end{itemize}
%
%\subsubsection*{Architectures}
%TensorFlow and Keras are popular deep learning frameworks created and supported by Google. Both are static computation graph frameworks, which means that a model's structure and dataflow are defined ahead of time and cannot be modified during runtime. Conversely, PyTorch is a dynamic computation graph framework, which means that the architecture of the model can be changed during runtime. Models that we wanted to create were either all inherently static graphs, or we could easily implement the dynamic nature of the computation with some creative engineering. Out of the three, Keras presents a very straightforward and concise API, although it comes with a learning curve. All of these points made a good argument in favor of Keras, but PyTorch was also familiar since its API is straightforward and ``Pythonic". TensorFlow, which Keras can use as a backend, presented an API that is verbose in many ways, especially when creating deep models that stack many layers. Since Keras can directly work with TensorFlow when needed, we preferred to use Keras where possible.
%
%\subsubsection*{GPU acceleration}
%TensorFlow and Keras both provide simple, built-in libraries to use GPU acceleration for training models. With limited boilerplate and infrastructure setup, all GPU acceleration is abstracted away from the user. While this abstraction makes TensorFlow and Keras extremely easy to use, it takes away all fine control from the user if they wish to control their own GPU memory usage. Furthermore, PyTorch provides the ability to the user to define which portions of code will use the GPU. This makes it more complicated to provide acceleration, but allows the user to granularly control GPU usage. In addition, Keras, TensorFlow, and PyTorch all provide transparent APIs to utilize multiple GPUs to enable massive data parallelization.
%
%\vspace{5pt}

Overall, Keras provided us the flexibility and ease of use that we required. The custom functions that we wanted to implement were not overly complicated, and with some careful thinking and working within the framework's constraints, we would be able to create the functionality required. Furthermore, a baseline model provided by \cite{Christie2017} was also implemented in Keras, providing us an easy reference to base our code on. We heavily considered PyTorch but preferred the plug-and-play nature of Keras instead. Had we approached this problem with complex, novel architectures, PyTorch would have been the preferred choice.


==> SymlinkSubsection.tex <==
\subsubsection{Use symlinks where possible}
Keras provides a built in data loading utility called \textit{ImageDataGenerator}\footnote{https://keras.io/preprocessing/image/}. However, \textit{ImageDataGenerator} requires a fixed directory structure, which caused us to move data around to different directory structures depending on the data pipeline. Moving data is an operation that takes time dependent on the underlying storage medium, filesystem, and size of the data itself. Ideally, moving data should be limited as much as possible so time is not wasted, but in certain cases, it is unavoidable. In this use case, we incurred frequent moves of every image up and down the directory structure. It would have taken considerable engineering to recreate the functionality of \textit{ImageDataGenerator} to fit our directory structure, so we decided to use symlinks to create an efficient way to move data around.

By using symlinks, we created an ephemeral file and directory structure that could be manipulated rapidly without shuffling entire images around. Although this method still incurred some disk latency, we were able to move entire symlinks in large blocks, providing us a {\raise.17ex\hbox{$\scriptstyle\sim$}}4x speedup compared to moving entire images around.

==> SystemSpecSubsection.tex <==
\subsection{Infrastructure Limitations and Solutions}
As a small research and prototyping lab, the CMU SEI Emerging Technology Center has general purpose hardware that is reconfigured and utilized for many different tasks as needed. To accommodate the FMoW challenge's unique and large computational requirements on our varied compute infrastructure, we identified and engineered clever trade-offs that provided significant boosts to our performance.

\subsubsection{System Specification}
\begin{figure}[h]
	\includegraphics[width=2.5in, height=1.4in]{IARPAInfrastructure.png}
	\caption{Simplified infrastructure diagram.}
	\label{fig:Infrastructure}
\end{figure}

All data storage, processing, and learning was done on two servers that the CMU SEI self-hosts. Since most machines in our computing lab are multi-tenant, we identified these two servers to be single-tenant for the duration of the competition. We will refer to these machines as GPU-CLUSTER and STR-CLUSTER, for a general-purpose GPU compute cluster and storage server, respectively. Mainly used for deep learning applications, GPU-CLUSTER is a fast, compute-heavy server that lacks a large amount of storage. STR-CLUSTER is a large storage server meant to hold and transfer data over the network and is not meant for large compute operations. Since this problem required both a large computational load as well as large storage requirements, a careful interfacing of these two systems was necessary.

\vspace{10pt}
\textbf{GPU-CLUSTER:}
\begin{itemize}
	\item CPU: 2x Intel\textregistered{} Xeon\textregistered{} E5-2640 v4 @ 2.40GHz
	\item Memory: 8x 32GB (256GB) DDR4-2400MHz ECC
	\item Storage: 2x Intel\textregistered{} SSD 240GB, 2.5in SATA 6Gb/s, RAID 1 (HW)
	\item GPU: 8x Nvidia GeForce GTX 1080 (8GB GDDR5X, 2560 CUDA cores)
\end{itemize}
{\addtolength{\leftskip}{4mm}
\textbf{STR-CLUSTER:}
\begin{itemize}
	\item CPU: 2x Intel\textregistered{} Xeon\textregistered{} E5620 @ 2.40GHz
	\item Memory: 12x 8GB (96GB)
	\item Storage: 8x Intel HDD 2TB, RAID 6 (HW)
\end{itemize}
}
\vspace{10pt}

STR-CLUSTER and GPU-CLUSTER are connected via an Ethernet switch. STR-CLUSTER has a 2x10 GbE connection to the switch in LACP mode, for an effective 20 GbE data pipe. However, GPU-CLUSTER has a 10 GbE connection to the switch, meaning the overall system has an effective max throughput of 10 GbE (See Figure \ref{fig:Infrastructure}).

\subsubsection{Slow writes and deletes}
Our storage server was set up to be a general-purpose, read-operation oriented server. With deep learning tasks that include heavy data augmentation and image processing with frequent temporary file writes, this is not an ideal setup. Existent hardware RAID 6, also known as double-parity RAID due to its use of two parity stripes on each disk, on STR-CLUSTER, presented a significant challenge as RAID 6 is not meant to be used in a heavy write setup. Due to existent data on the server that was not removable, we had to identify and work around many limitations of this system.

STR-CLUSTER was mounted on GPU-CLUSTER via an NFS mount. The RAID 6 hard drive setup, high hard disk latency, and less-than-ideal network bandwidth usage resulted in slow random create and delete operations.
\begin{figure}[h]
	\includegraphics[width=3in, height=2.25in]{DiskLatency.png}
	\caption{Disk latency on random access creates, reads, and deletes.}
	\label{fig:DiskLatency}
\end{figure}
While random creates and deletes were at an unacceptable threshold (see Figure \ref{fig:DiskLatency}, random reads were at a reasonable level. We decided to take full advantage of our highly performant random reads and created a system to work around our high create workload. By creating a 100 GB RAM disk on GPU-CLUSTER, we were able to stream data from STR-CLUSTER into the RAM disk via sequential block reads (which were {\raise.17ex\hbox{$\scriptstyle\sim$}}100x lower latency), perform heavy creates on RAM disk, and almost instantly delete the relevant files. With careful engineering and tuning, we developed a system to seamlessly stream files and get a speedup of {\raise.17ex\hbox{$\scriptstyle\sim$}}5x on our overall filesystem operations.
